SCW Codes for Maximum Likelihood Detection in Diffusive Molecular Communications without Channel State Information

Instantaneous or statistical channel state information (CSI) is needed for most detection schemes developed for molecular communication (MC) systems. Since the MC channel changes over time, e.g., due to variations in the velocity of flow, the temperature, or the distance between transmitter and receiver, CSI acquisition has to be conducted repeatedly to keep track of CSI variations. Frequent CSI acquisition may entail a large overhead whereas infrequent CSI acquisition may result in a low CSI estimation accuracy. To overcome these challenges, we design codes which enable maximum likelihood sequence detection at the receiver without instantaneous or statistical CSI. In particular, assuming concentration shift keying modulation, we show that a class of codes, referred to as strongly constant-weight (SCW) codes, enables optimal CSI-free sequence detection at the expense of a decrease in data rate. For the proposed SCW codes, we analyze the code rate, the error rate, and the average number of released molecules. In addition, we study the properties of binary SCW codes and balanced SCW codes in further detail. Simulation results verify our analytical derivations and reveal that SCW codes with CSI-free detection outperform uncoded transmission with optimal coherent and non-coherent detection.

==> Fig/BER_K/BER_K.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{012}[cl][cl]{\matlabtextA Sub-Optimal CSI-Free Detector (Uncoded Transmission) [9]}%
\psfrag{013}[cl][cl]{\matlabtextA Optimal Coherent Detector (Uncoded Transmission) [7]}%
\psfrag{014}[cl][cl]{\matlabtextA Optimal Non-Coherent Detector (Uncoded Transmission) [9]}%
\psfrag{015}[cl][cl]{\matlabtextA Proposed Optimal CSI-Free Detector (Coded Transmission)}%
\psfrag{016}[cl][cl]{\matlabtextA $R=[\frac{1}{2},\frac{1}{3},\frac{1}{4}]$}%
\psfrag{017}[bc][bc]{\matlabtextA BER}%
\psfrag{018}[tc][tc]{\matlabtextA Codeword/Block Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $2$}%
\psfrag{001}[ct][ct]{\matlabtextA $4$}%
\psfrag{002}[ct][ct]{\matlabtextA $6$}%
\psfrag{003}[ct][ct]{\matlabtextA $8$}%
\psfrag{004}[ct][ct]{\matlabtextA $10$}%
\psfrag{005}[ct][ct]{\matlabtextA $12$}%
\psfrag{006}[ct][ct]{\matlabtextA $14$}%
\psfrag{007}[ct][ct]{\matlabtextA $16$}%
\psfrag{008}[ct][ct]{\matlabtextA $18$}%
\psfrag{009}[ct][ct]{\matlabtextA $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{-1}$}%
%
%% </ytick>

==> Fig/CER_SCW/CER_SCW.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[5,0,1]^{\mathsf{T}}$}%
\psfrag{011}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[3,0,3]^{\mathsf{T}}$}%
\psfrag{012}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[1,2,3]^{\mathsf{T}}$}%
\psfrag{013}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[3,2,1]^{\mathsf{T}}$}%
\psfrag{014}[cl][cl]{\matlabtextA $\bar{\boldsymbol{\omega}}=[2,2,2]^{\mathsf{T}}$}%
\psfrag{015}[cl][cl]{\matlabtextA Upper Bounds}%
\psfrag{016}[cl][cl]{\matlabtextA Analytical}%
\psfrag{017}[cl][cl]{\matlabtextA Results}%
\psfrag{018}[cl][cl]{\matlabtextA Simulation}%
\psfrag{019}[bc][bc]{\matlabtextA CER}%
\psfrag{020}[tc][tc]{\matlabtextA SINR (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
\psfrag{004}[ct][ct]{\matlabtextA $25$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/CER_SCW_Bal/CER_SCW_Bal.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextA $L=6$}%
\psfrag{012}[cl][cl]{\matlabtextA $L=4$}%
\psfrag{013}[cl][cl]{\matlabtextA $L=3$}%
\psfrag{014}[cl][cl]{\matlabtextA $L=2$}%
\psfrag{015}[bc][bc]{\matlabtextA CER}%
\psfrag{016}[tc][tc]{\matlabtextA SINR (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
\psfrag{004}[ct][ct]{\matlabtextA $25$}%
\psfrag{005}[ct][ct]{\matlabtextA $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/CER_SNR/CER_SNR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{008}[cl][cl]{\matlabtextA Lower Bound (Proposition 3)}%
\psfrag{009}[cl][cl]{\matlabtextA Upper Bound (Proposition 3)}%
\psfrag{010}[cl][cl]{\matlabtextA Upper Bound (Corollary 3)}%
\psfrag{011}[cl][cl]{\matlabtextA Upper Bound (Proposition 2)}%
\psfrag{012}[cl][cl]{\matlabtextA Simulation}%
\psfrag{013}[cl][cl]{\matlabtextA Full Binary CW Code}%
\psfrag{014}[cl][cl]{\matlabtextA with Rate $R=0.5$}%
\psfrag{015}[cl][cl]{\matlabtextA Binary CW Code}%
\psfrag{016}[bc][bc]{\matlabtextA CER}%
\psfrag{017}[tc][tc]{\matlabtextA SINR (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{003}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{004}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{0}$}%
%
%% </ytick>

==> Fig/RateK/RateK.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA Asymptotic Result}%
\psfrag{018}[cl][cl]{\matlabtextA Upper Bound}%
\psfrag{019}[cl][cl]{\matlabtextA Lower Bound}%
\psfrag{020}[cl][cl]{\matlabtextA Exact Code Rate}%
\psfrag{021}[cl][cl]{\matlabtextA $\rho=1/4$}%
\psfrag{022}[cl][cl]{\matlabtextA $\rho=1/3$}%
\psfrag{023}[cl][cl]{\matlabtextA $\rho=1/2$}%
\psfrag{024}[bc][bc]{\matlabtextA Code Rate, $R^{\mathrm{code}}(K,\omega)$}%
\psfrag{025}[tc][tc]{\matlabtextA Codeword Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $20$}%
\psfrag{002}[ct][ct]{\matlabtextA $40$}%
\psfrag{003}[ct][ct]{\matlabtextA $60$}%
\psfrag{004}[ct][ct]{\matlabtextA $80$}%
\psfrag{005}[ct][ct]{\matlabtextA $100$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.55$}%
\psfrag{008}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{009}[rc][rc]{\matlabtextA $0.65$}%
\psfrag{010}[rc][rc]{\matlabtextA $0.7$}%
\psfrag{011}[rc][rc]{\matlabtextA $0.75$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.85$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.9$}%
\psfrag{015}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{016}[rc][rc]{\matlabtextA $1$}%
%
%% </ytick>

==> Fig/RateKmulti/RateKmulti.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{016}[cl][cl]{\matlabtextA Asymptotic Result}%
\psfrag{017}[cl][cl]{\matlabtextA $L=8$ with $\boldsymbol{\rho}=\frac{1}{16}[4,3,2,2,2,1,1,1]^{\mathsf{T}}$}%
\psfrag{018}[cl][cl]{\matlabtextA $L=8$ with $\boldsymbol{\rho}=\frac{1}{8}[1,1,1,1,1,1,1,1]^{\mathsf{T}}$}%
\psfrag{019}[cl][cl]{\matlabtextA $L=4$ with $\boldsymbol{\rho}=\frac{1}{8}[4,2,1,1]^{\mathsf{T}}$}%
\psfrag{020}[cl][cl]{\matlabtextA $L=4$ with $\boldsymbol{\rho}=\frac{1}{4}[1,1,1,1]^{\mathsf{T}}$}%
\psfrag{021}[bc][bc]{\matlabtextA Code Rate, $R^{\mathrm{code}}(\bar{\boldsymbol{\omega}})$}%
\psfrag{022}[tc][tc]{\matlabtextA Codeword Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $50$}%
\psfrag{002}[ct][ct]{\matlabtextA $100$}%
\psfrag{003}[ct][ct]{\matlabtextA $150$}%
\psfrag{004}[ct][ct]{\matlabtextA $200$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{006}[rc][rc]{\matlabtextA $0.55$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{008}[rc][rc]{\matlabtextA $0.65$}%
\psfrag{009}[rc][rc]{\matlabtextA $0.7$}%
\psfrag{010}[rc][rc]{\matlabtextA $0.75$}%
\psfrag{011}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.85$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.9$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{015}[rc][rc]{\matlabtextA $1$}%
%
%% </ytick>

==> Fig/RateL/RateL.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{020}[cl][cl]{\matlabtextA $K=[2,4,6,8,10,12,16,18,20,24,30,32,36,40]$}%
\psfrag{021}[bc][bc]{\matlabtextA Code Rate, $R^{\mathrm{code}}(\bar{\boldsymbol{\omega}})$}%
\psfrag{022}[tc][tc]{\matlabtextA Number of Symbols, $L$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
\psfrag{004}[ct][ct]{\matlabtextA $20$}%
\psfrag{005}[ct][ct]{\matlabtextA $25$}%
\psfrag{006}[ct][ct]{\matlabtextA $30$}%
\psfrag{007}[ct][ct]{\matlabtextA $35$}%
\psfrag{008}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{010}[rc][rc]{\matlabtextA $0.55$}%
\psfrag{011}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.65$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.7$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.75$}%
\psfrag{015}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{016}[rc][rc]{\matlabtextA $0.85$}%
\psfrag{017}[rc][rc]{\matlabtextA $0.9$}%
\psfrag{018}[rc][rc]{\matlabtextA $0.95$}%
\psfrag{019}[rc][rc]{\matlabtextA $1$}%
%
%% </ytick>

==> Fig/RateLinf/RateLinf.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[cl][cl]{\matlabtextA $K=[2,4,6,8,10,12,16,18,20,24,30,32,36,40]$}%
\psfrag{018}[bc][bc]{\matlabtextA Data Rate, $R^{\mathrm{inf}}(\bar{\boldsymbol{\omega}})$}%
\psfrag{019}[tc][tc]{\matlabtextA Number of Symbols, $L$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
\psfrag{004}[ct][ct]{\matlabtextA $20$}%
\psfrag{005}[ct][ct]{\matlabtextA $25$}%
\psfrag{006}[ct][ct]{\matlabtextA $30$}%
\psfrag{007}[ct][ct]{\matlabtextA $35$}%
\psfrag{008}[ct][ct]{\matlabtextA $40$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{010}[rc][rc]{\matlabtextA $1$}%
\psfrag{011}[rc][rc]{\matlabtextA $1.5$}%
\psfrag{012}[rc][rc]{\matlabtextA $2$}%
\psfrag{013}[rc][rc]{\matlabtextA $2.5$}%
\psfrag{014}[rc][rc]{\matlabtextA $3$}%
\psfrag{015}[rc][rc]{\matlabtextA $3.5$}%
\psfrag{016}[rc][rc]{\matlabtextA $4$}%
%
%% </ytick>

==> Fig/Tradeoff_CER/Tradeoff_CER.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{009}[cl][cl]{\matlabtextA MPPM, $\omega=2$}%
\psfrag{010}[cl][cl]{\matlabtextA PPM, $\omega=1$}%
\psfrag{011}[cl][cl]{\matlabtextA Unbalanced, $\omega=K/4$}%
\psfrag{012}[cl][cl]{\matlabtextA Balanced, $\omega=K/2$}%
\psfrag{013}[bc][bc]{\matlabtextA b)}%
\psfrag{014}[bc][bc]{\matlabtextA CER}%
\psfrag{015}[tc][tc]{\matlabtextA Codeword Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
\psfrag{004}[ct][ct]{\matlabtextA $25$}%
\psfrag{005}[ct][ct]{\matlabtextA $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-1}$}%
%
%% </ytick>

==> Fig/Tradeoff_Energy/Tradeoff_Energy.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{014}[bc][bc]{\matlabtextA c)}%
\psfrag{015}[bc][bc]{\matlabtextA Normalized Number of Released Molecules, $\bar{N}^{\mathrm{tx}}_{\mathrm{nrm}}(K,\omega)$}%
\psfrag{016}[tc][tc]{\matlabtextA Codeword Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
\psfrag{004}[ct][ct]{\matlabtextA $25$}%
\psfrag{005}[ct][ct]{\matlabtextA $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{008}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{009}[rc][rc]{\matlabtextA $0.3$}%
\psfrag{010}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.7$}%
%
%% </ytick>

==> Fig/Tradeoff_Rate/Tradeoff_Rate.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{017}[bc][bc]{\matlabtextA a)}%
\psfrag{018}[bc][bc]{\matlabtextA Data Rate, $R^{\mathrm{inf}}(K,\omega)$}%
\psfrag{019}[tc][tc]{\matlabtextA Codeword Length, $K$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $5$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $15$}%
\psfrag{003}[ct][ct]{\matlabtextA $20$}%
\psfrag{004}[ct][ct]{\matlabtextA $25$}%
\psfrag{005}[ct][ct]{\matlabtextA $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.1$}%
\psfrag{008}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{009}[rc][rc]{\matlabtextA $0.3$}%
\psfrag{010}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{011}[rc][rc]{\matlabtextA $0.5$}%
\psfrag{012}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{013}[rc][rc]{\matlabtextA $0.7$}%
\psfrag{014}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{015}[rc][rc]{\matlabtextA $0.9$}%
\psfrag{016}[rc][rc]{\matlabtextA $1$}%
%
%% </ytick>
